ScalaBFS: A Scalable BFS Accelerator on HBM-Enhanced FPGAs

High Bandwidth Memory (HBM) provides massive aggregated memory bandwidth by exposing multiple memory channels to the processing units. To achieve high performance, an accelerator built on top of an FPGA configured with HBM (i.e., FPGA-HBM platform) needs to scale its performance according to the available memory channels. In this paper, we propose an accelerator for BFS (Breadth-First Search) algorithm, named as ScalaBFS, that builds multiple processing elements to sufficiently exploit the high bandwidth of HBM to improve efficiency. We implement the prototype system of ScalaBFS and conduct BFS in both real-world and synthetic scale-free graphs on Xilinx Alveo U280 FPGA card real hardware. The experimental results show that ScalaBFS scales its performance almost linearly according to the available memory pseudo channels (PCs) from the HBM2 subsystem of U280. By fully using the 32 PCs and building 64 processing elements (PEs) on U280, ScalaBFS achieves a performance up to 19.7 GTEPS (Giga Traversed Edges Per Second). When conducting BFS in sparse real-world graphs, ScalaBFS achieves equivalent GTEPS to Gunrock running on the state-of-art Nvidia V100 GPU that features 64-PC HBM2 (twice memory bandwidth than U280).

==> backup_system.tex <==
0\section{System Design}\label{sec:systemoverview}
We present the architecture of ScalaBFS, which consists of multiple \emph{Processing Groups} (PGs), an \emph{Scheduler}, and a \emph{Vertex dispatcher}. A PG consists of an \emph{HBM reader} and one or more \emph{Processing Elements} (PEs). A \emph{Scheduler} controls the execution of BFS. The HBM reader is employed by  all the PEs in the same PG to issue the read command to read the neighbor lists from the HBM. \emph{Vertex dispatcher} gathers all responses of neighbor lists from the HBM and then scatters the vertices in the neighbor lists to the PEs according to their vertex IDs (denoted as $VID$).
%The architecture of ScalaBFS is illustrated in Figure \ref{fig:architecture}. The accelerator consists of multiple \emph{Processing Groups} (PGs), each of which contains one \emph{HBM reader} and one or more \emph{Processing Elements} (PEs); A \emph{Scheduler} that controls the execution of BFS; A \emph{Vertex dispatcher} that gathers all responses of neighbor lists from the HBM and then scatters the vertices in the neighbor lists to the PEs according to their vertex IDs (denoted as $VID$).

\begin{figure}[t]
	\centering
 	\setlength{\abovecaptionskip}{+5pt}
 	\setlength{\belowcaptionskip}{-15pt}
	\includegraphics[width = 3in]{./figures/fig2-system-arch.pdf}	
	\caption{Architecture of ScalaBFS}
	\label{fig:architecture}
\end{figure}

\begin{figure*}[t]
	\centering
	%\setlength{\abovecaptionskip}{+1pt}
	%\setlength{\belowcaptionskip}{-12pt}	
	\begin{subfigure}{.16\textwidth}
		\centering
		\includegraphics[width=1\linewidth]{./figures/fig3-examp-graph-a.pdf}
		\caption{example graph}
		\label{subfig:example}
	\end{subfigure}%
	\hfill
	\begin{subfigure}{.28\textwidth}
		\centering
		\includegraphics[width=1\linewidth]{./figures/fig3-examp-graph-b.pdf}
		\caption{CSR \& CSC}
		\label{subfig:csrcsc}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.28\textwidth}
		\centering
		\includegraphics[width=1\linewidth]{./figures/fig3-examp-graph-c.pdf}
		\caption{two subgraphs}
		\label{subfig:patitioned}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.2\textwidth}
		\centering
		\includegraphics[width=1\linewidth]{./figures/fig3-examp-graph-d.pdf}
		\caption{adj. matrix view}
		\label{subfig:matrix}
	\end{subfigure}
	\caption{Partitioning an example graph into two subgraphs.}
	\label{fig:partitionexamplegraph}
\end{figure*}

Each PG is assigned exclusively to a single HBM pseudo channel (PC), and its HBM reader issues memory requests to its corresponding HBM PC via AXI port. Therefore, ScalaBFS has no more than 32 PGs on Xilinx Alveo U280, as its HBM subsystem has only 32 PCs (shown in Figure \ref{fig:u280hbm}). Each PE of ScalaBFS is in charge of processing an \emph{interval} of vertices of an input graph. By this, if ScalaBFS has $Q$ PEs, the vertex ID space of an input graph is divided into $Q$ non-overlapping intervals. For load balancing among the PEs, the vertex IDs are hashed before assigning to the intervals, such that the $i^{th}$ PE is in charge of processing the vertices whose $VID \% Q = i$. The PEs work in hybrid (push-pull) processing mode according to the stages of BFS, to improve the bandwidth utilization rate.

Similar to \cite{Wang:2010} and \cite{Lei:2015}, ScalaBFS uses the on-chip memory resources (i.e., BRAMs and URAMs) that are distributedly attached to the PEs to store all the vertex data. There are several reasons behind this design choice: 1) In ScalaBFS, we want to investigate the upper-bound performance on BFS that an FPGA card can achieve. Storing the vertex data in the on-chip memory resources can greatly reduce the number of memory accesses towards the off-chip memory devices, and thus reveal the real potential of FPGAs on conducting BFS. 2) FPGAs now have larger and larger storage capacity in both BRAM and URAM. When carefully designed, a modern data center accelerator card like U280 can process graphs with millions of vertices by using its on-chip memories.

In the following discussions, we will first explain how ScalaBFS places the data in subsection \ref{subsec:dataplacement}, then elaborate the design of the PEs in subsection \ref{subsec:hybridpe}, and discuss the design of HBM reader and Vertex dispatcher in subsection \ref{subsec:readeranddispatcher}.

\subsection{Data Placement}\label{subsec:dataplacement}

For an input graph, we separate its data into two types: the vertex data and graph data. The vertex data refer to the level array, while the graph data refer to the neighbor lists. As shown in Algorithm \ref{alg:bfs-general}, during the execution of BFS, the vertex data are frequently changed to track the status (i.e., active or visited) of vertices, and at the same time, store the result level values. On the contrary, the graph data never change. With these facts, ScalaBFS employs different strategies to handle them: for vertex data, ScalaBFS uses bitmaps stored in the BRAM to track the status changing, and allocates URAM space to store the result level values temporarily. For graph data, ScalaBFS partitions them into multiple subgraphs and stores them in the HBM PCs. 

\subsubsection{Vertex data}

We define three bitmaps, i.e., \emph{current frontier}, \emph{next frontier} and \emph{visited map}, to track the statuses of vertex data during the execution of BFS, and each vertex occupies a single bit from each of these bitmaps (a vertex thus consumes 3 bits, totally). These three bitmaps are stored in double pump BRAMs, such that two operations can be conducted on them within a clock cycle. A bit in the current frontier indicates whether its corresponding vertex is active (1 for active, and 0 for inactive) in the current iteration. Similarly, a bit in the next frontier indicates whether its corresponding vertex will be activated in the next iteration. The bits in the visited map indicate whether their corresponding vertices are visited before (1 for visited, and 0 for un-visited). Algorithm \ref{alg:bfs-optimize} lists the new BFS algorithm by using these three bitmaps. 

\begin{algorithm}[h]
	\caption{BFS algorithm using three bitmaps}
	\label{alg:bfs-optimize}
 	\setlength{\abovecaptionskip}{+5pt}
	\setlength{\belowcaptionskip}{-15pt}	
	\Input{Directed graph $G$, and \texttt{root} vertex $r$.}
	\Output{Array $Level[0...|V|-1]$, distances of vertices from $r$.}
	\DontPrintSemicolon
	\ForEach{$i\in [0,|V|-1]$}{
		$Level[i] \gets \infty$; $current\_frontier[i] \gets 0$; \\
		$next\_frontier[i] \gets 0$; $visited\_map[i] \gets 0$; \\
	}
	$Level[r] \gets 0$; $bfs\_level \gets 0$;\\
	$current\_frontier[r] \gets 1$; $visited\_map[r] \gets 1$;\\
	
	\tcp*[l]{push mode (beginning and ending iterations).}
	\While{$\exists i \in V$, such that $current\_frontier[i]=1$ } {
		\ForEach{vertex $i$ whose $current\_frontier[i]=1$}{
			\ForEach{outgoing neighbour $v$ of $i$}{
				\If{$visited\_map[v] == 0$}{
					$next\_frontier[v] \gets 1$;\\
					$visited\_map[v] \gets 1$;\\
					$Level[v] \gets bfs\_level + 1$;
				}
			}
		}
		$bfs\_level \gets bfs\_level + 1$; \\
		$swap(current\_frontier, next\_frontier)$
	}
	
	\tcp*[l]{pull mode (mid-term iterations).}
	\While{$\exists i \in V$, such that $visited\_map[i]\neq1$ } {
		\ForEach{vertex $i$ whose $visited\_map[i]\neq1$}{
			\ForEach{incoming neighbour $u$ of $i$}{
				\If{$current\_frontier[v] == 1$}{
					$next\_frontier[i] \gets 1$;\\
					$visited\_map[i] \gets 1$;\\
					$Level[i] \gets bfs\_level + 1$;
				}
			}
		}
		$bfs\_level \gets bfs\_level + 1$; \\
		$swap(current\_frontier, next\_frontier)$
	}
\end{algorithm}

During a push mode iteration, the current frontier is scanned to locate all the active vertices. And then for each active vertex, vertices in its outgoing (child) neighbor list will be checked. If a vertex in the list is not visited before (by checking the visited map), its corresponding bit in the visited map and next frontier will be set, and its level value will be written back to the level array stored in URAMs. Whereas during a pull mode iteration, the visited map will be scanned to locate all unvisited vertices. And then for each unvisited vertex, vertices in its incoming (parent) neighbor list will be checked. If a parent vertex in the list is active (by checking the current frontier), the corresponding bits in the visited map and next frontier of the aforementioned unvisited vertex will be set, and its level value will be written back to URAMs. 

\begin{figure*}[ht]
	\centering
	%\setlength{\abovecaptionskip}{+1pt}
	\setlength{\belowcaptionskip}{-10pt}	
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width=1\linewidth]{./figures/fig4-hybrid-pe-push.pdf}
		\caption{push mode}
		\label{subfig:pushmode}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.45\textwidth}
		\centering
		\includegraphics[width=1\linewidth]{./figures/fig4-hybrid-pe-pull.pdf}
		\caption{pull mode}
		\label{subfig:pullmode}
	\end{subfigure}
	\caption{Processing logic for push mode and pull mode.}
	\label{fig:hybridpipelines}
\end{figure*}

\subsubsection{Graph data}

We use Compressed Sparse Row (CSR) and its transpose, i.e., Compressed Sparse Column (CSC), to represent the graph data. The CSR consists of an offset array and an edge array, where the offset array stores the offsets of the outgoing (child) neighbor lists. The CSC has a similar structure as CSR, except that its edge array stores the incoming (parent) neighbor lists. The reason for ScalaBFS to use both CSR and CSC is that they facilitate the PEs to obtain both the outgoing and incoming neighbor lists of a selected vertex. Figure \ref{fig:partitionexamplegraph} gives an example graph and its CSR and CSC representations.

Suppose there are two PEs, and the vertex ID space of the example graph in Figure \ref{subfig:example} is divided into two intervals, i.e., [0,2,4] and [1,3,5], due to the load-balancing reason. We partition the graph data according to the partitioning results on the vertex ID space: neighbor lists of the vertices belonging to the same partition will be placed in the same subgraph as shown in Figure \ref{subfig:patitioned}. From the viewpoint of the adjacency matrix, our partitioning scheme partitions a graph \emph{horizontally}, which is different from \cite{Finnerty:2019} where the input graph is partitioned vertically. The reason for this horizontal partition scheme is that it does not breakdown the neighbor lists, and longer neighbor lists mean more chances of sequential accesses towards the HBM, which helps on improving the memory bandwidth usage rates during processing. 

In ScalaBFS, the number of PEs decides the number of subgraphs. In the above example, if the two PEs belong to two different PGs, the two subgraphs will be stored in two different HBM PCs, assigned to the two PGs respectively. Whereas, if both PEs belong to the same PG, the two subgraphs will be stored in the same HBM PC. 

\begin{figure*}[ht]
	\centering
	%\setlength{\abovecaptionskip}{+1pt}
	\setlength{\belowcaptionskip}{-10pt}	
	\begin{subfigure}{.28\textwidth}
		\centering
		\includegraphics[width=0.9\linewidth]{./figures/fig5-crossbars-fullcrossbar.pdf}
		\caption{full crossbar}
		\label{subfig:fullcrossbar}
	\end{subfigure}%
	\hfill
	\begin{subfigure}{.65\textwidth}
		\centering
		\includegraphics[width=0.9\linewidth]{./figures/fig5-crossbars-2layercrossbar.pdf}
		\caption{equivalent 2-layer crossbar}
		\label{subfig:2layercrossbar}
	\end{subfigure}
	\caption{Converting full-crossbar into multi-layer crossbar.}
	\label{fig:crossbar}
\end{figure*}

\subsection{Hybrid Mode PE}\label{subsec:hybridpe}

To efficiently use the available memory bandwidth, the processing elements (PEs) in ScalaBFS employ a hybrid processing mode: they work in the push mode for beginning and ending iterations, and work in the pull mode during the mid-term iterations as listed in Algorithm \ref{alg:bfs-optimize}. The Scheduler in Figure \ref{fig:architecture} decides the processing mode of the PEs, and informs its decisions to the PEs at the start of each iteration during the fly. 

Figure \ref{fig:hybridpipelines} illustrates the processing logic for these two processing modes. From Figure \ref{fig:hybridpipelines}, we can observe that the functionalities of these two processing modes are similar, and both of them can be divided into three processing stages: 

$\bullet$ \textbf{Workload preparing (P1)}

This stage prepares the workloads to be processed. When working in the push mode, the active vertices are first obtained from the current frontier, and then passed to the \emph{Read CSR} module to read their outgoing neighbor lists from the CSR data. As the CSR data are stored in HBM, the module will pass its requests to the HBM reader. When working in the pull mode, the unvisited vertices are obtained from the visited map, and the remaining processes are the same as in the push mode except that the \emph{Read CSC} module will read the CSC data for incoming neighbor lists from the HBM. 

$\bullet$ \textbf{Neighbor checking (P2)}

This stage accepts messages (i.e., the neighboring vertices) from the Vertex dispatcher. When working in the push mode, the messages will be the outgoing (child) neighbors of the active vertices prepared by the stage of P1. For each child vertex, the processing logic will proceed to check the visited map, and pass it to the next stage of processing (i.e., P3) if it is not visited before, or drop it if otherwise. When working in the pull mode, the messages will be the incoming (parent) neighbors of the unvisited vertices prepared by the stage of P1. For each parent vertex, the processing logic will then proceed to check the current frontier, and pass \emph{its child vertex} (i.e., the unvisited vertex prepared by the stage P1) to the next stage of processing (i.e., P3) if it (the parent vertex) is active, or drop it if otherwise. 

Note that in the pull mode, the child vertex to be passed to stage P3 may \emph{not} be in the same PE as that processing its parent, since the incoming neighbor lists in CSC contains vertices of other partitions as shown in Figure \ref{subfig:patitioned}. In such a case, the child vertex will be passed from one PE to another PE via a soft crossbar, which will be discussed in detail in the next subsection. 

$\bullet$ \textbf{Result writing (P3)}

This stage accepts result messages from P2 and conducts the modifications in the bitmaps according to Algorithm \ref{alg:bfs-optimize}. In both processing modes, the results will be written to the next frontier and visited map. Besides, the results will also be written to the Level array stored in the URAM (not shown in Figure \ref{fig:hybridpipelines} for brevity). 

Due to the similarities of the logic for these two processing modes, except for the soft crossbar used in P2 in the pull processing mode, we use the same sets of circuits with parameters in registers to implement the similar modules, to save logic resources of the FPGA. Moreover, as the above processing stages are driven by signals (from the Scheduler) or data streams from other modules, the circuits work asynchronously in a pipeline fashion to maximize the efficiency of processing.

\subsection{HBM reader and Vertex dispatcher}\label{subsec:readeranddispatcher}

In ScalaBFS, the functionality of an HBM reader is simple: it receives requests from the \emph{Read CSR} or \emph{Read CSC}, converts the requests into memory accessing AXI commands, and issues them to its corresponding HBM PC. Suppose we are now working in the push mode, and a request (reading the outgoing neighbor list of an active vertex) is sent to an HBM reader. The HBM reader will first assemble an AXI command to read the corresponding values in the offset array of CSR from the HBM. After receiving the offset values, the HBM reader will then assemble another AXI command to read the outgoing neighbor list from the edge array. Procedures are similar for the pull mode, except that the offsets in the CSC and incoming neighbor lists are to be read. 

The neighbor lists read from the HBM are \emph{intercepted} by the Vertex dispatcher. The functionality of the Vertex dispatcher is to scrutinize the vertices in the input neighbor-list streams, classify them according to intervals that they belong to, and send them to the corresponding PEs. The most straightforward approach that achieves such an objective is to use a full $N\times N$ crossbar when there are $N$ PEs (and accordingly, $N$ subgraphs). However, such a full crossbar consumes $N^2$ FIFO resources \cite{Wang:2010}, which is hard for an FPGA to satisfy when $N$ scales to a relatively large number. For example, when defining the length of FIFO as 16 bytes and $N=64$, the Vertex dispatch using a full 64$\times$64 crossbar consumes more than half of the LUTs from U280 FPGA card, and thus limits the scalability. 

To reduce the logic resource consumption on Vertex dispatcher, we proposed a method that converts a full crossbar into a \emph{multi-layer crossbar}\footnote{We do not use more complex routing techniques like the torus network \cite{Lei:2015}, since the switching logic of our Vertex dispatcher is unidirectional (and thus simpler), and our multi-layer crossbar approach is easier for implementation.}. The method is inspired by previous works \cite{Ferreira:2011} on crossbars. To explain our method, we discuss a case that dispatches 16 neighbor-list streams to 16 PEs as shown in Figure \ref{fig:crossbar}. Figure \ref{subfig:fullcrossbar} depicts the 16$\times$16 full crossbar that contains 16 input and 16 output ports. The switching logic of this 16$\times$16 full crossbar is to send a vertex to the $(VID\%16)^{th}$ port, where $VID$ denotes the vertex's ID. 

Equivalently, we can convert the 16$\times$16 full crossbar into a two-layer crossbar, which consists of two layers (input layer and output layer) and each layer contains four 4$\times$4 crossbar, as shown in Figure \ref{subfig:2layercrossbar}. The switching logic of each 4$\times$4 crossbar of the input layer is to send a vertex to its $(VID\%4)^{th}$ port, which connects to the $(VID\%4)^{th}$ 4$\times$4 crossbar of the output layer. The $i^{th}$ 4$\times$4 crossbar of the output layer connects to the PEs such that $PE_{ID}\%4 = i$, where $PE_{ID}$ denotes the ID of a PE. By this for the output layer, the first ($0^{th}$) 4$\times$4 crossbar connects to $PE_0$, $PE_4$, $PE_8$ and $PE_{12}$, while the second ($1^{th}$) 4$\times$4 crossbar connects to $PE_1$, $PE_5$, $PE_9$ and $PE_{13}$, and so on. The switching logic of each 4$\times$4 crossbar of the output layer is thus to send an incoming vertex to the $(VID\%16)^{th}$ PE (equals to the effectiveness of the 16$\times$16 full crossbar). 

To generalize our approach on converting an $N\times N$ full crossbar into a multi-layer crossbar: we need first decompose $N$ into multiple (say $k$) factors, such that $N = C_1\times C_2 \times ... \times C_k$. The first (input) layer uses $N/C_1$ $C_1\times C_1$ crossbars, and classifies the input vertices into $C1$ groups according to $VID\%C_1$, where $VID$ denotes the ID of an input vertex. The second (relay) layer uses $N/C_2$ $C_2\times C_2$ crossbars, and further classifies the input vertices into $C1\times C2$ groups according to $VID\%(C_1 \times C2)$. Such process continues till the vertices arrive at the last (output) layer, which uses $N/C_k$ $C_k\times C_k$ crossbars, and classifies the vertices into $C_1\times C_2\times ... \times C_k = N$ groups. The ($N$) vertex groups coming out of the last layer are finally sent to the ($N$) PEs, each of which is in charge of processing one vertex group (i.e., a vertex interval). Figure \ref{fig:crossbar} merely illustrates a simple case where $N=16$, $k=2$, and $C_1=C_2=4$. 

We now compare these two approaches (full-crossbar vs. multi-layer crossbar) from the angles of resource consumption and efficiency. An $N\times N$ full crossbar consumes $N^2$ FIFOs, while the number of FIFOs required by its equivalent $k$-layer crossbar is $(N/C_1) \times C_1^2 + (N/C_2) \times C_2^2 + ... + (N/C_k) \times C_k^2$. It is easy to prove that the number of FIFOs consumed by our $k$-layer crossbar is smaller than that of its equivalent $N\times N$ full crossbar, as $N = C_1\times C_2 \times ... \times C_k$. Consider the example in Figure \ref{fig:crossbar}, the 16$\times$16 full crossbar consumes $16\times 16 = 256$ FIFOs, while the two-layer crossbar consume only $2\times 4\times 4\times4 = 128$ FIFOs, meaning half resource consumption. 

From the efficiency point of view, the $N\times N$ full-crossbar achieves 1-hop latency on message passing, while the equivalent $k$-layer crossbar approach requires k-hop latency for vertex dispatching. Obviously, the $k$-layer crossbar approach leads to higher latency than the full crossbar approach as $k\geq 2$. Nevertheless, based on the observation that BFS is a throughput-critical workload as discussed in subsection \ref{subsec:bfsalgorithm}, it is appropriate for us to use multi-layer crossbars to trade latency for resource. In Section \ref{sec:performance}, we will use 3-layer 4$\times$4 crossbars to replace the 64$\times$64 full crossbar to help our accelerator to achieve the scale of 64 PEs on U280. 

